Pay attention! - Robustifying a Deep Visuomotor Policy through Task-Focused Attention

Several recent studies have demonstrated the promise of deep visuomotor policies for robot manipulator control. Despite impressive progress, these systems are known to be vulnerable to physical disturbances, such as accidental or adversarial bumps that make them drop the manipulated object. They also tend to be distracted by visual disturbances such as objects moving in the robot's field of view, even if the disturbance does not physically prevent the execution of the task. In this paper, we propose an approach for augmenting a deep visuomotor policy trained through demonstrations with Task Focused visual Attention (TFA). The manipulation task is specified with a natural language text such as `move the red bowl to the left'. This allows the visual attention component to concentrate on the current object that the robot needs to manipulate. We show that even in benign environments, the TFA allows the policy to consistently outperform a variant with no attention mechanism. More importantly, the new policy is significantly more robust: it regularly recovers from severe physical disturbances (such as bumps causing it to drop the object) from which the baseline policy, i.e. with no visual attention, almost never recovers. In addition, we show that the proposed policy performs correctly in the presence of a wide class of visual disturbances, exhibiting a behavior reminiscent of human selective visual attention experiments. Our proposed approach consists of a VAE-GAN network which encodes the visual input and feeds it to a Motor network that moves the robot joints. Also, our approach benefits from a teacher network for the TFA that leverages textual input command to robustify the visual encoder against various types of disturbances.

==> future_work.tex <==
\section{Future work}
\label{sec:Future}
In general, paying attention to more important parts of an image or video, results in faster reaction and less computation. Moreover, attention can really show its strength when it has been used in cluttered environments. It is not feasible and/or practical for a network to be able to perform the requested task in presence of arbitrary objects, which the network didn't see in the training samples. Attention can help the network ignore irrelevant parts of the environment and focus on what has been requested from it. One interesting future direction is to perform tasks in a cluttered environment without a significant drop in it's performance.
